Optimal and Learning Control for Autonomous Robots

Optimal and Learning Control for Autonomous Robots has been taught in the Robotics, Systems and Controls Masters at ETH Zurich with the aim to teach optimal control and reinforcement learning for closed loop control problems from a unified point of view. The starting point is the formulation of of an optimal control problem and deriving the different types of solutions and algorithms from there. These lecture notes aim at supporting this unified view with a unified notation wherever possible, and a bit of a translation help to compare the terminology and notation in the different fields. The course assumes basic knowledge of Control Theory, Linear Algebra and Stochastic Calculus.

==> OLCAR_Chapter.03.tex <==
\chapter{Path Integrals}

%
\section{The Brownian Motion}
Brownian motion, or random walk, is defined as a stochastic process of some variable, $w$, with a Gaussian probability
distribution as follows
%
\begin{equation} \label{eq:brownian_motion_pdf} 
\mathbb{P}_{\textbf{w}}(t,w) = \frac{1}{\sqrt{2 \pi \sigma^2 t}} \exp{\left(- \frac{(w-\mu t)^2}{2 \sigma^2 t} \right)}
\end{equation}
%
At each instance in time, this process has a Gaussian distribution with the following mean
and variance:
%
\begin{align}
&\mathbb{E} \{w(t)\} = \mu t \notag \\
&\mathbb{V}ar \{w(t)\} = \sigma^2 t 
\end{align}
%
To define the probability distribution of a stochastic process, we need to
define not only $P_{\textbf{w}}(t,w)$ but also the joint distribution of the
stochastic process for an arbitrary subset of time steps i.e.
$P_{\textbf{w}}(t_1,w_1,\dots,,t_N,w_N)$.

Instead of defining the joint probability distribution directly, we will define the
Brownian motion's increment process, $ dw(t) = \lim\limits_{\Delta t \to 0}{w(t + \Delta t) - w(t)}$ by the two
following characteristics:
%
\begin{enumerate}
\item The increment process, $dw(t)$, has a Gaussian distribution with the
mean and the variance, $\mu \Delta t$ and $\sigma^2 \Delta t$ respectively.
\item The increment process, $dw(t)$, is statistically independent of
$w(s)$ for all $s \leq t$.
\end{enumerate}
%
With these characteristics of the increment process and the probability distribution introduced
in equation~\eqref{eq:brownian_motion_pdf}, we can derive the joint distribution of any arbitrary set of time instances. For example, we can show that the joint distribution for $w(t)$ and
$w(s)$ is a Gaussian distribution with the cross covariance
%
\begin{equation*}
\mathbb{E}{ \left\{\left( w(t)-\mu t \right) \left( w(s) - \mu s \right) \right\} } = \sigma^2 \min(t,s)
\end{equation*}
%
Figure \ref{fig:brownian_motion} illustrates 15 samples extracted from a Brownian
motion with $\mu=5$ and $\sigma^2 = 4$ within a time period [0 2]. An interesting
aspect of Brownian motion is that even though it is continuous over time,
it is not differentiable.
%
\begin{figure} [h]
\centering
\includegraphics[width=0.6\textwidth]{browian_motion}
\caption{Brownian Motion with $\mu = 5$ and $\sigma^2 = 4$}
\label{fig:brownian_motion}
\end{figure}

In order to simulate the Brownian motion, either we should find the joint probability
distribution of $\{ w(0), w(\Delta t), w(2\Delta), \dots, w(N \Delta t) \}$
and then extract samples from it or we should forward integrate the following equation
(which is in fact a discretized stochastic differential equation)
%
\begin{equation*}
w(t+\Delta t) = w(t) + \mu \Delta t + \sqrt{\Delta t \sigma^2} \varepsilon, \qquad w(0) = 0
\end{equation*}
%
where $\varepsilon$ is extracted from a normal distribution with zero mean and
variance one. In this equation, the terms $\mu \Delta t + \sqrt{\Delta t \sigma^2}
\varepsilon$ are used to approximate the increment process, $dw$. In the limit
when $\Delta t$ approaches to zero, this term will be equal to the increment
process. Throughout this chapter we will mostly use the increment process instead of the Brownian motion itself.

Finally, the Brownian motion can be easily extended to n-dimension vector form as
%
\begin{equation*}
\mathbb{P}_{\textbf{w}}(t,\vw) = \frac{1}{(2\pi)^{n/2} (\mathbf{\Sigma} t)^{1/2}} \exp{\left(- \frac{1}{2}(\vw-\vmu t)^T (\mathbf{\Sigma} t)^{-1} (\vw-\mathbf{\vmu} t) \right)}
\end{equation*}
%

%
\section{Stochastic Differential Equations}
The following equation describes a Stochastic Differential Equation (SDE)
%
\begin{equation} \label{eq:sde_equation}
d\vx = \vf(t,\vx)dt + \vg(t,\vx) d\vw
\end{equation}
%
where $\vx(t)$ is a stochastic vector process of dimension $n$ and $\vw(t)$ is a
Brownian motion with zero mean and identity covariance matrix ($d\vw$ is the
increment process). $\vf(t,\vx)$ and  $\vg(t,\vx)$ are called respectively the
drift and the diffusion coefficients. Note that for $ \vg(t,\vx) = \mathbf{0}$
the SDE reduces to the well-known Ordinary Differential Equation (ODE).
Furthermore defining the mean and covariance of the Brownian motion to zero and
the identity matrix, respectively, is not a restrictive assumption. Since any
arbitrary Brownian motion can be put in this form by adding the mean
to the drift coefficient and multiplying the diffusion coefficient by the square
root of the covariance matrix.

One simple approach for simulating the SDE in equation~\eqref{eq:sde_equation} is to
discretize it over time by some sufficiently small time step $\Delta t$ and
replace $d\vw$ by $\sqrt{\Delta t} \varepsilon$. In doing this, we assume
that during the time step $\Delta t$ the Brownian motion has a constant increment
with mean zero and covariance $\Delta t \vI$. The discretized SDE is then expressed as follows:
%
\begin{equation} \label{eq:sde_equation_discretized}
\vx(t_{n+1}) = \vx(t_n) + \vf(t_n,\vx(t_n))\Delta t + \vg(t_n,\vx(t_n)) \sqrt{\Delta t}
\varepsilon,  \qquad \varepsilon \sim \mathcal{N}(\mathbf{0},\vI)
\end{equation}
%
Note that when equation~\eqref{eq:sde_equation} is non-linear, as is typically the case,
$\vx$ will have a non-Gaussian distribution. However the following conditioned
probability distribution for an infinitely small time step is always Gaussian.
%
\begin{equation} \label{sde_conditioned_pdf}
\mathbb{P}_{\textbf{x}}(t+\Delta t,\vx \mid t, \vy) = \mathcal{N} \Big( \vy + \vf(t,\vy)\Delta t, \vg(t,\vy) \vg^T(t,\vy) \Delta t\Big)
\end{equation}
%


%
\section{The Fokker Planck Equation} \label{sec:fokker_planck_equation}
Consider the SDE in equation~\eqref{eq:sde_equation}. Despite the fact that the Brownian
motion has a Gaussian distribution, generally the resulting process does not have
a Gaussian distribution (except in the linear case). However the probability
distribution associated to the SDE in equation~\eqref{eq:sde_equation} can be
derived as a solution to an initial value Partial Differential Equation (PDE)
known as Fokker Plank equation.

We define $\mathbb{P}_{\textbf{x(t)}}(t ,\vx \mid s, \vy)$ as the conditioned
probability distribution of $x(t)$ knowing that the process at time $s$ has
value $\vy$ ($\vx(s) = \vy$). The governing PDE on this probability
distribution is defined by the following Fokker Planck equation
%
\begin{equation} \label{eq:fokker_planck_equation}
\partial_t\mathbb{P} = -\nabla_x^T (\vf\mathbb{P}) + \cfrac{1}{2} \operatorname{Tr}{\left[\nabla_{xx} (\vg \vg^T \mathbb{P})\right]}
\end{equation}
%
with initial condition $\mathbb{P}_{\textbf{x(t)}}(t=s ,\vx \mid s, \vy) = \delta(\vx-\vy)$.
The operators $\nabla_x()$ and $\nabla_{xx}()$ are defined as:
%
\begin{equation*}
\nabla_x() = \begin{bmatrix} \frac{\partial}{\partial x_1} \\ \frac{\partial}{\partial x_2} \\ \vdots \\ \frac{\partial}{\partial x_n} \end{bmatrix}   \qquad \qquad
\nabla_{xx}() = 
\begin{bmatrix} 
\frac{\partial}{\partial x_{11}}  & \dots & \frac{\partial}{\partial x_{1n}} \\
\vdots & \ddots & \vdots \\
\frac{\partial}{\partial x_{n1}}  & \dots & \frac{\partial}{\partial x_{nn}}
\end{bmatrix}
\end{equation*}
%
where $x_{i}$ is the \textit{i}th element of the n-dimension stochastic process vector $\vx$.


%
\section{Linearly-Solvable Markov Decision Process}  \label{sec:LMDP}
The Linearly-Solvable Markov Decision Process (LMDP) is a class of optimal control
problems in which the optimality equation (characterized by the Bellman equation or
the HJB equation) can be transformed into a linear form. In this section we will
consider a special case of this class with stochastic dynamics defined as follows
%
\begin{equation}  \label{eq:LMDP_sde}
d\vx = \vf(t,\vx) dt + \vg(t,\vx) \left(\vu dt + d\vw\right), \qquad d\vw \sim \mathcal{N}(\mathbf{0},\mathbf{\Sigma}dt)
\end{equation}
%
where $\vx$ is the state vector of size $n$, $\vu$ is the control input of
size $m$, and $\vw$ is the $m$-dimension Brownian motion with zero mean and
covariance $\mathbf{\Sigma} dt$. In the control literature, the system described
by equation~\eqref{eq:LMDP_sde} is called a control affine system since the
control input appears linearly in the differential equations. Note that if we
divide the both  sides of the equation by $dt$, and then substitute
$\frac{d\vw}{dt}$ for $\vvep$ (stationary white noise), we get a system
equation in the class of systems introduced in \sref{subsec:HJP_fin_sto}
(equation~\ref{eq:stochastic_cont_time_system_eq}).
%
\begin{equation*}
\dot{\vx} = \vf(t,\vx) + \vg(t,\vx) \left(\vu + \vvep\right), \qquad \vvep \sim \mathcal{N}(\mathbf{0},\mathbf{\Sigma})
\end{equation*}
%
The cost function for this optimal control problem is defined as
%
\begin{equation} \label{eq:LMDP_cost}
J = E \left\{\Phi(\vx(t_f))+ \int_{t_0}^{t_f} {q(t,\vx) + \frac{1}{2} \vu^T \vR \vu \ dt} \right\}
\end{equation}
%
The expectation is over the trajectories extracted from the stochastic process
described by equation~\eqref{eq:LMDP_sde}. The only difference between this cost
function and the general one introduced by
equation~\eqref{eq:stochastic_continuous_time_deterministic cost function} is
that the control input cost is quadratic.

In order to make this optimal control problem a LMDP, we need to add another 
condition which is
%
\begin{equation} \label{eq:LMDP_condition}
\vR \mathbf{\Sigma} = \lambda \vI
\end{equation}
%
where $\lambda$ is an arbitrary positive real number. This condition has the following
intuitive interpretation: Let's assume for simplicity that both $\mathbf{\Sigma}$ and
$\vR$ are diagonal matrices. Then we get
%
\begin{equation*}
\vR_{ii} \mathbf{\Sigma}_{ii} = \lambda, \qquad \text{\textit{for all }} i \in \{1,\dots,m\}
\end{equation*}
%
This means that if the covariance of the noise affecting control input $i$ is
relatively high, the cost for that control input should be lower. Higher control
effort should be tolerated to counteract the noise (note that in
equation~\ref{eq:LMDP_sde} the process noise is added to the control input).

Now we will show how the optimal control problem can be transformed to
an LMDP. We will start by writing the HJB equation for this problem. We will use
the HJB equation given in equation~\eqref{eq:stchastic_principle_of_optimality}
with the following substitutions
%
\begin{eqnarray}	
\beta \leftarrow 0 \hspace{50mm} \notag  & & L(\vx, \vu(t)) \leftarrow q(t,\vx) + \frac{1}{2} \vu^T \vR \vu  \notag \\
\vf_t (\vx,\vu(t)) \leftarrow \vf(t,\vx) + \vg(t,\vx) \vu  \hspace{10mm} \notag & & \vB(t) \leftarrow \vg(t,\vx) \notag \\
\vW(t) \leftarrow \mathbf{\Sigma} \hspace{43mm} \notag & &
\end{eqnarray}
%
Then we get
%
\begin{equation} \label{eq:LMDP_HJB}
- \partial_t V^*(t,\vx) = \min_{\vu} \left\{q(t,\vx) + \frac{1}{2} \vu^T \vR \vu + \nabla_x^T V^*(t,\vx) (\vf(t,\vx) + \vg(t,\vx) \vu) + \frac{1}{2} \mathtt{Tr} [\nabla_{xx} V^*(t,\vx) \vg(t,\vx) \mathbf{\Sigma} \vg^T(t,\vx)]  \right\}
\end{equation}
%
where $V^*$ is the optimal value function. For simplicity, we will omit all the
dependencies with respect to time and state. In equation~\eqref{eq:LMDP_HJB} we
have also adopted the notation introduced in \sref{sec:fokker_planck_equation}. If we
minimize the left hand side with respect to $\vu$, we get
%
\begin{equation} \label{eq:LMDP_HJB_minimized}
- \partial_t V^* = q - \frac{1}{2} \nabla_x^T V^* \, \vg \vR^{-1} \! \vg^T \nabla_x V^* + \nabla_x^T V^* \, \vf + \frac{1}{2} \mathtt{Tr} [\nabla_{xx} V^* \, \vg \mathbf{\Sigma} \vg^T]
\end{equation}
%
and the optimal control
%
\begin{equation}
\vu^*(t,\vx) = - \vR^{-1} \vg^T(t,\vx) \nabla_x V(t,\vx) 
\end{equation} 
%
Equation~\eqref{eq:LMDP_HJB_minimized} is a nonlinear PDE, since $\nabla_x^T V^*$
appears in a quadratic form. In order to shorten the notion, we substitute $\vg \,
\vR^{-1} \! \vg^T$ by $\mathbf{\Xi}$. Using the
condition~\ref{eq:LMDP_condition}, we can also write $\vg \mathbf{\Sigma} \vg^T =
\lambda \mathbf{\Xi}$. Therefore
%
\begin{equation} \label{eq:LMDP_HJB_main}
- \partial_t V^* = q - \frac{1}{2} \nabla_x^T V^* \, \mathbf{\Xi} \nabla_x V^* + \nabla_x^T V^* \, \vf + \frac{\lambda}{2} \mathtt{Tr} [\nabla_{xx} V^* \, \mathbf{\Xi}]
\end{equation}
%
In spite of the nonlinearity of the resulting equation, it can be shown that
under a log transformation we get a linear PDE. Assume the following
transformation $\Psi(t,\vx)$ is called the desirability function
%
\begin{equation} \label{eq:log_transform}
V^*(t,\vx) = - \lambda \log{\Psi(t,\vx)},
\end{equation}
%
we can write the derivatives as 
%
\begin{eqnarray} \label{eq:log_transform_derivatives}
\partial_t V^*(t,\vx) & = & - \lambda \frac{\partial_t \Psi}{\Psi} \notag \\
\nabla_x V^*(t,\vx) & = & - \lambda \frac{\nabla_x \Psi}{\Psi} \notag \\
\nabla_{xx} V^*(t,\vx) & = & \frac{1}{\lambda} \nabla_x V^* \: \nabla_x^T V^* - \lambda \frac{\nabla_{xx} \Psi}{\Psi}.
\end{eqnarray}
%
Furthermore, for the scalar value $-\frac{1}{2} \nabla_x^T V^* \, \mathbf{\Xi}
\nabla_x V^*$ in equation~\eqref{eq:LMDP_HJB_main} we can write
%
\begin{equation} \label{eq:log_transform_Tr}
-\frac{1}{2} \nabla_x^T V^* \, \mathbf{\Xi} \nabla_x V^* = -\frac{1}{2} \mathtt{Tr} [\nabla_x^T V^* \, \mathbf{\Xi} \nabla_x V^*] = -\frac{1}{2} \mathtt{Tr} [\nabla_x V^* \, \nabla_x^T V^* \, \mathbf{\Xi}].
\end{equation}
%
By substituting equations~\eqref{eq:log_transform_derivatives} and \eqref{eq:log_transform_Tr} into equation~\eqref{eq:LMDP_HJB_main}, we get
%
\begin{equation*}
\lambda \frac{\partial_t \Psi}{\Psi} = q - \cancel{\frac{1}{2} \mathtt{Tr} [\nabla_x V^* \, \nabla_x^T V^* \, \mathbf{\Xi}]} - \lambda \vf^T \frac{\nabla_x \Psi}{\Psi} + \cancel{\frac{1}{2} \mathtt{Tr} [\nabla_x V^* \, \nabla_x^T V^* \, \mathbf{\Xi}]} - \frac{\lambda^2}{2} \mathtt{Tr} \left[ \frac{\nabla_{xx} \Psi}{\Psi} \mathbf{\Xi} \right].
\end{equation*}
%
Finally, we multiply both sides by $-\sfrac{\Psi}{\lambda}$
%
\begin{equation} \label{eq:LMDP_pde}
- \partial_t \! \Psi = -\frac{1}{\lambda} q \Psi +  \vf^T \nabla_x \! \Psi + \frac{\lambda}{2} \mathtt{Tr} [ \mathbf{\Xi} \nabla_{xx} \! \Psi ].
\end{equation}
%
Note that we used the matrix identity $\mathtt{Tr}[\vA \vB] = \mathtt{Tr}[\vB
\vA]$ to write $\mathtt{Tr} [ \nabla_{xx} \! \Psi \, \mathbf{\Xi}  ] =
\mathtt{Tr} [ \mathbf{\Xi} \nabla_{xx} \! \Psi ]$. Equation~\eqref{eq:LMDP_pde}
is linear with respect to $\Psi$ and its derivatives. This equation is normally
written in the form of the linear operator $\mathtt{H}$ as follows
%
\begin{equation} \label{eq:LMDP_pde_short}
- \partial_t \! \Psi = \mathtt{H} [\Psi]
\end{equation}
%
where $\mathtt{H}$ is defined as
%
\begin{align} \label{eq:LMDP_H_operator}
\mathtt{H} &= -\frac{1}{\lambda} q +  \vf^T \nabla_x + \frac{\lambda}{2} \mathtt{Tr} [ \mathbf{\Xi} \nabla_{xx}] \notag \\ 
&= -\frac{1}{\lambda} q + \sum_{i}{\vf_i \frac{\partial \;}{\partial_{x_i}}} + \frac{\lambda}{2} \sum_{i,j}{\mathbf{\Xi}_{ij} \frac{\partial^2 \quad}{\partial_{x_i} \partial_{x_j}}}
\end{align}
%
From the principle of optimality, we know that the original optimal control problem is a final value problem, meaning that only the terminal condition is known prior to solving. Equation~\eqref{eq:LMDP_pde} is therefore also a final value problem, which has the following
terminal value.
%
\begin{align} \label{eq:LMDP_pde_terminal_value}
\Psi(t_f,\vx) &= \exp \left(-\frac{1}{\lambda} V^*(t_f,\vx) \right) \notag \\
&= \exp \left(-\frac{1}{\lambda} \Phi(\vx) \right)
\end{align}
%
The equation~\eqref{eq:LMDP_pde_short} is consider to be an LMDP. In the next
section, we will introduce the Path Integral method to solve this PDE.

%
\section{Path Integral Optimal Control}
The Path Integral framework introduces a method for solving the linear backward PDE
introduced in equation~\eqref{eq:LMDP_pde_short} through a forward integration
approach. We start the proof by introducing a new function over time and state, 
$\rho(t,\vx)$. We also define the following inner product in the function space which 
is in fact a function of time.
%
\begin{equation}
<\rho \mid \Psi> = \int{\rho(t,\vx) \Psi(t,\vx) d\vx}
\end{equation}
%
We also assume that 
%
\begin{equation} \label{eq:rho_inifine_condition}
\lim\limits_{\norm{x} \to \infty}{\rho(t,\vx) = 0}
\end{equation}
%
The $\mathtt{H}^\dagger$ operator is called the Hermitian conjugate of the
operator $\mathtt{H}$ (equation_\ref{eq:LMDP_H_operator}) if it satisfies the
following equality.
%
\begin{equation}
<\rho \mid \mathtt{H} [\Psi]> = <\mathtt{H}^\dagger [\rho] \mid \Psi>
\end{equation}
%
The $\mathtt{H}^\dagger$ formulation can be derived as follows by starting from the definitions of the inner product and the $\mathtt{H}$ operator.
%
\begin{align}
<\rho \mid \mathtt{H} [\Psi]> &= \int{\rho(t,\vx) \mathtt{H} [\Psi(t,\vx)] d\vx}  \notag \\
&= \int{\rho(t,\vx) \, \left(-\frac{1}{\lambda} q + \sum_{i}{\vf_i \frac{\partial \;}{\partial_{x_i}}} + \frac{\lambda}{2} \sum_{i,j}{\mathbf{\Xi}_{ij} \frac{\partial^2 \quad}{\partial_{x_i} \partial_{x_j}}}\right) \Psi(t,\vx) d\vx}
\end{align}
%
Using integration by parts and the assumption in \ref{eq:rho_inifine_condition} 
we can easily show
%
\begin{align*}
<\rho \mid \mathtt{H} [\Psi]> &= \int{\Psi \left(-\frac{1}{\lambda} q \rho - \sum_{i}{ \frac{\partial \left( \vf_i \rho \right)}{\partial_{x_i}}} + \frac{\lambda}{2} \sum_{i,j}{ \frac{\partial^2 \left(\mathbf{\Xi}_{ij} \rho \right) }{\partial_{x_i} \partial_{x_j}}} \right)  d\vx} \\ 
&= \int{\Psi(t,\vx) \mathtt{H}^\dagger [\rho(t,\vx)] d\vx}
\end{align*}
%
Therefore we can write $\mathtt{H}^\dagger$ as
%
\begin{align}
\mathtt{H}^\dagger &= -\frac{1}{\lambda} q - \sum_{i}{ \frac{\partial \vf_i }{\partial_{x_i}}} + \frac{\lambda}{2} \sum_{i,j}{ \frac{\partial^2 \mathbf{\Xi}_{ij} }{\partial_{x_i} \partial_{x_j}}} \notag \\
&= -\frac{1}{\lambda} q - \nabla_x^T \vf + \frac{\lambda}{2} \mathtt{Tr} [ \nabla_{xx} \mathbf{\Xi}]
\end{align}
%
So far the only restriction that we have posed over $\rho(t,\vx)$ is the
condition~\ref{eq:rho_inifine_condition}. We will now pose another restriction on
$\rho(t,\vx)$ that $<\rho \mid \Psi>$ is time independent. Therefore we have
%
\begin{equation}
\frac{d \ }{dt} <\rho \mid \Psi> = 0
\end{equation}
%
Then we can write
%
\begin{align*}
0 &=\frac{d \ }{dt} <\rho \mid \Psi> \\
&= \int{\partial_t \Big(\rho(t,\vx) \Psi(t,\vx)\Big) d\vx} \\
&= \int{\partial_t \rho(t,\vx) \Psi(t,\vx) + \rho(t,\vx) \partial_t \Psi(t,\vx) d\vx} \\
&= <\partial_t \rho \mid \Psi> + <\rho \mid \partial_t \Psi> 
\end{align*}
%
By using the equation~\eqref{eq:LMDP_pde_short}, we get
%
\begin{equation*}
0 = <\partial_t \rho \mid \Psi> - <\rho \mid \mathtt{H} [\Psi]> 
\end{equation*}
%
Now we use the Hermitian conjugate operator $\mathtt{H}^\dagger$
%
\begin{equation*}
0 = <\partial_t \rho \mid \Psi> - <\mathtt{H}^\dagger[\rho] \mid \Psi> 
\end{equation*}
%
Therefore we can write
%
\begin{equation*}
<\partial_t \rho - \mathtt{H}^\dagger[\rho] \mid \Psi> = 0
\end{equation*}
%
A trivial solution to this equation is 
%
\begin{align} \label{eq:forward_diffusion_process_pdf}
\partial_t \rho &= \mathtt{H}^\dagger[\rho] \notag \\
&= -\frac{1}{\lambda} q \rho - \nabla_x^T (\vf \rho) + \frac{\lambda}{2} \mathtt{Tr} [ \nabla_{xx} (\mathbf{\Xi} \rho)]
\end{align}
%
Since equation~\eqref{eq:LMDP_pde_short} is a final value problem,
equation~\eqref{eq:forward_diffusion_process_pdf} should be an initial value
problem, otherwise the terminal value for $\rho$ cannot be defined freely, as the
inner product should be time independent. 

Furthermore it can be shown that if $\rho(t,\vx)$ satisfies the
equation~\eqref{eq:forward_diffusion_process_pdf}, it will always satisfy the
condition in \ref{eq:rho_inifine_condition}. Therefore by only determining the
initial value, we can uniquely define a $\rho(t,\vx)$ function which satisfies all
of the conditions. In the literature this equation is sometimes referred to as a
forward diffusion process. 

We will now define an appropriate
initial condition for this forward diffusion process. Equation~\eqref{eq:forward_diffusion_process_pdf} resembles the Fokker Planck
equation (equation~\ref{eq:fokker_planck_equation}). The only difference is the
term $-\frac{1}{\lambda} q \rho$. The effect of this extra term is that the probability
distribution decays over time. Based on this similarity, we can show that the
following process has the same probability distribution as the solution of
equation~\eqref{eq:forward_diffusion_process_pdf} (note that we are misusing the
term ``probability distribution''. As mentioned the term $-\frac{1}{\lambda} q
\rho$ attenuates the probability distribution over time, therefore its
integral eventually becomes less than one).
%
\begin{align} \label{eq:forward_diffusion_process_sde}
& d\vx(t_i) = \vf(t_i,\vx(t_i)) dt + \vg(t_i,\vx(t_i)) d\vw, \qquad \vx(t_0 = s) = \vy \notag \\
& \begin{cases}
\vx(t_{i+1}) = \vx(t_i) + d\vx(t_i) \quad \text{with probability } \exp \left(-\frac{1}{\lambda} q dt\right) \\
\vx(t_{i+1}): \text{annihilation} \hspace{9.5mm} \text{with probability } 1-\exp \left(-\frac{1}{\lambda} q dt\right)
\end{cases}
\end{align}
%
where $\vw$ is a Brownian motion with zero mean and the covariance
$\mathbf{\Sigma} dt$ and $t_{i+1} = t_i + dt$. Here ``annihilation'' means that
we discard the sample with some probability. Through the similarity to
the Fokker Planck equation, we also can determine an appropriate initial condition. If
the state vector at time $s$ is $\vy$ then the probability distribution of the state
at the initial time should be a delta function at $\vy$.
%
\begin{equation} \label{eq:forward_diffusion_process_initial}
\rho(t=s,\vx) = \delta(\vx - \vy)
\end{equation}
%
In order to emphasize that the $\rho(t,\vx)$ is a solution to the diffusion
process with the initial condition $\vx(s) = \vy$, sometimes the initial
condition is explicitly written in the condition i.e. we write $\rho(t,\vx\mid s, \vy)$.

Since the process described by equation~\eqref{eq:forward_diffusion_process_sde}
is a Markov Process we can write the joint probability distribution of a
trajectory $\tau = \{ \vx(t_{0}), \vx(t_{1}), \dots \vx(t_{N}) \}$, with $t_0 = s$, as
%
\begin{equation}
\rho(\tau \mid s,\vy) = \prod\limits_{i=0}^{N-1} {\rho(t_{i+1},\vx(t_{i+1}) \mid t_{i},\vx(t_{i}))}, \qquad \vx(t_0=s) = \vy
\end{equation}
%
where $N$ is the number of the time steps and the initial state at time $s$ is
$\vy$. Furthermore the conditioned probability distribution will have a Gaussian
like distribution.
%
\begin{equation} 
\rho(t_{i+1},\vx(t_{i+1}) \mid t_{i},\vx(t_{i})) = \operatorname{e}^{-\frac{1}{\lambda} q(t_i,\vx(t_i)) dt} \mathcal{N} \Big(\vx(t_i) + \vf(t_i,\vx(t_i)) dt, \mathbf{\Xi}(t_i,\vx(t_i)) dt \Big)
\end{equation}
%
Here $\mathbf{\Xi}(t_i,\vx(t_i))$ is defined as \sref{sec:LMDP}. The effect of
the annihilation process is incorporated by multiplying the distribution by
$\exp{(-\frac{1}{\lambda} q dt)}$. Therefore the probability distribution of the
trajectory $\tau$ can be written as
%
\begin{align} \label{eq:forward_diffusion_process_tau_pdf}
\rho(\tau \mid s,\vy) &= \prod\limits_{i=0}^{N-1} {\operatorname{e}^{-\frac{1}{\lambda} q(t_i,\vx(t_i)) dt} \mathcal{N} \Big(\vx(t_i) + \vf(t_i,\vx(t_i)) dt, \mathbf{\Xi}(t_i,\vx(t_i)) dt \Big)} \notag \\
&= \operatorname{e}^{\sum\limits_{i=0}^{N-1}{-\frac{1}{\lambda} {q(t_i,\vx(t_i)) dt}}} \ \prod\limits_{i=0}^{N-1} {\mathcal{N} \Big(\vx(t_i) + \vf(t_i,\vx(t_i)) dt, \mathbf{\Xi}(t_i,\vx(t_i)) dt \Big)}   \notag \\
=& \mathbb{P}_{uc}(\tau \mid s, \vy) \ \operatorname{e}^{\sum\limits_{i=0}^{N-1}{-\frac{1}{\lambda} {q(t_i,\vx(t_i)) dt}}}
\end{align}
%
where $\mathbb{P}_{uc}(\tau \mid s, \vy)$ is introduced in
equation~\eqref{eq:LMDP_tau_pdf} and it is actually the probability distribution
of the trajectory $\tau$ generated by the system in
equation~\eqref{eq:forward_diffusion_process_sde} \textbf{without the
annihilation} when initialized at $\vx(s) = \vy$. Furthermore by omitting the
annihilation term from equation~\eqref{eq:forward_diffusion_process_sde}, it will
reduce to the same system as LMDP (equation~\ref{eq:LMDP_sde}) when the $\vu$ is
set to zero. In control literature such a system is normally referred to as the
uncontrolled system (hence the subscript ``\textit{uc}'').
%
\begin{equation} \label{eq:LMDP_tau_pdf}
\mathbb{P}_{uc}(\tau \mid s, \vy) = \prod\limits_{i=0}^{N-1} {\mathcal{N} \Big(\vx(t_i) + \vf(t_i,\vx(t_i)) dt, \mathbf{\Xi}(t_i,\vx(t_i)) dt \Big)}
\end{equation}
%
Now we go back to the characteristic that the inner product of $\Psi(t,\vx)$ and
$\rho(t,\vx)$ is time independent. Since the inner product is time independent,
its value at any time will be always the same. Therefore for the initial
time and the final time we can write
%
\begin{align}
<\rho \mid \Psi>(t=s) &= <\rho \mid \Psi>(t=t_f) \notag \\
\int{\rho(s,\vx_s) \Psi(s,\vx_s) d\vx_s} &= \int{\rho(t_f,\vx_{t_f}) \Psi(t_f,\vx_{t_f}) d\vx_{t_f}}
\end{align}
%
By substituting the initial condition given in
equation~\eqref{eq:forward_diffusion_process_initial} and integrating it we will
get
%
\begin{align}
\int{\delta(\vx_s-\vy) \Psi(s,\vx_s) d\vx_s} &= \int{\rho(t_f,\vx_{t_f}) \Psi(t_f,\vx_{t_f}) d\vx_{t_f}} \notag \\
\Psi(s,\vy) &= \int{\rho(t_f,\vx_{t_f}) \Psi(t_f,\vx_{t_f}) d\vx_{t_f}} \notag
\end{align}
%
Now we will use the terminal condition of $\Psi$ from equation~\eqref{eq:LMDP_pde_terminal_value}.
%
\begin{equation*}
\Psi(s,\vy) = \int{\rho(t_f,\vx_{t_f}) \operatorname{e}^{-\frac{1}{\lambda} \Phi(\vx_{t_f})} d\vx_{t_f}} 
\end{equation*}
%
To calculate the RHS integral we need to define the probability distribution at the last time step $t_f$. We can derive $\rho(t_f,\vx_{t_f})$ by marginalizing the joint probability distribution introduced in equation~\eqref{eq:forward_diffusion_process_tau_pdf} with respect to $\{ \vx(t_{1}), \dots \vx(t_{N-1}) \}$. Note that the time index starts from $t_1$ and goes up to $t_{N-1}$. 
%
\begin{align*}
\rho(t_f,\vx_{t_f}) &= \int{\rho(\tau \mid s,\vy) \, d\vx(t_1) \dots \vx(t_{N-1})} \\
&= \int{ \mathbb{P}_{uc}(\tau \mid s, \vy) \ \operatorname{e}^{\sum\limits_{i=0}^{N-1}{-\frac{1}{\lambda} {q(t_i,\vx(t_i)) dt}}} \ d\vx(t_1) \dots d\vx(t_{N-1})}
\end{align*}
%
By substituting this in the previous equation, we get (we have changed the name of $\vx_{t_f}$ to $\vx(t_{N})$)
%
\begin{equation}
\Psi(s,\vy) = \int{ \mathbb{P}_{uc}(\tau \mid s, \vy) \ \operatorname{e}^{-\frac{1}{\lambda}  \Big( \Phi(x(t_{N})) + \sum\limits_{i=0}^{N-1}{{q(t_i,\vx(t_i)) dt}} \Big) } \ d\vx(t_1) \dots d\vx(t_{N-1}) d\vx(t_{N}) }
\end{equation}
%
This equation is equal to the following expectation
%
\begin{align}
\Psi(s,\vy) &= \operatorname{E}_{\tau_{uc}} \left\{ \operatorname{e}^{-\frac{1}{\lambda}  \Big( \Phi(\vx(t_N)) + \sum\limits_{i=0}^{N-1}{{q(t_i,\vx(t_i)) dt}} \Big) } \right\} \notag \\
&= \operatorname{E}_{\tau_{uc}} \left\{ \operatorname{e}^{-\frac{1}{\lambda}  \Big( \Phi(\vx(t_f))+ \int_{s}^{t_f} {q(t,\vx) \ dt} \Big) } \right\}
\end{align}
%
where the first equation is the discretized equivalent of the latest one. We can
estimate this expectation through a Monte Carlo method by extracting samples and averaging them. The samples of this expectation are generated through the
uncontrolled dynamics system
%
\begin{equation}  \label{eq:uc_sde}
d\vx = \vf(t,\vx) dt + \vg(t,\vx) d\vw, \qquad d\vw \sim \mathcal{N}(\mathbf{0},\mathbf{\Sigma}dt), \quad \vx(t=s) = \vy
\end{equation}
%
Therefore in order to estimate the desirability function at time $s$ and state
$\vy$, we should forward simulate the uncontrolled dynamics several times with
the initial condition $\vx(s)=\vy$. Then we can estimate the expectation by
averaging the value of $-\frac{1}{\lambda}  \Big( \Phi(\vx(t_f))+ \int_{s}^{t_f}
{q(t,\vx) \ dt} \Big) $ for each sample.

After calculating the desirability function for all times and states, we can
derive the optimal control input as
%
\begin{align}
\vu^*(s,\vy) &= - \vR^{-1} \vg^T(s,\vy) \nabla_y V^*(s,\vy) \notag \\
&= \lambda \vR^{-1} \vg^T(s,\vy) \frac{\nabla_y \Psi(s,\vy)}{\Psi(s,\vy)}
\end{align} 
%
However we can also calculate the optimal control input directly by a similar
path integral approach
%
\begin{equation} \label{eq:pi_original_optimal_controller}
\vu^*(s,\vy) = \lim\limits_{\Delta s \to 0}{ \frac{  \operatorname{E}_{\tau_{uc}} \left\{ \displaystyle\int_{s}^{s+\Delta s} \!\!\!\!\! d\vw \  \operatorname{e}^{-\frac{1}{\lambda}  \Big( \Phi(\vx(t_f))+ \int_{s}^{t_f} {q(t,\vx) \ dt} \Big) } \right\} }    {\Delta s \operatorname{E}_{\tau_{uc}} \left\{ \operatorname{e}^{-\frac{1}{\lambda}  \Big( \Phi(\vx(t_f))+ \int_{s}^{t_f} {q(t,\vx) \ dt} \Big) } \right\}} }
\end{equation} 
%
again if we use the white noise notation where $\frac{d\vw}{dt} = \varepsilon$, we can write
%
\begin{equation} \label{eq:pi_optimal_controller}
\vu^*(s,\vy) = \frac{  \operatorname{E}_{\tau_{uc}} \left\{ \varepsilon \  \operatorname{e}^{-\frac{1}{\lambda}  \Big( \Phi(\vx(t_f))+ \int_{s}^{t_f} {q(t,\vx) \ dt} \Big) } \right\} }    {\operatorname{E}_{\tau_{uc}} \left\{ \operatorname{e}^{-\frac{1}{\lambda}  \Big( \Phi(\vx(t_f))+ \int_{s}^{t_f} {q(t,\vx) \ dt} \Big) } \right\}}
\end{equation} 
%
or equivalently 
%
\begin{equation} \label{eq:pi_optimal_controller1}
\vu^*(s,\vy) = \operatorname{E}_{\tau_{uc}} \left\{ \varepsilon \frac{  \operatorname{e}^{-\frac{1}{\lambda}  \Big( \Phi(\vx(t_f))+ \int_{s}^{t_f} {q(t,\vx) \ dt} \Big) }  }    {\operatorname{E}_{\tau_{uc}} \left\{ \operatorname{e}^{-\frac{1}{\lambda}  \Big( \Phi(\vx(t_f))+ \int_{s}^{t_f} {q(t,\vx) \ dt} \Big) } \right\}} \right\}
\end{equation} 
%
The samples are generated by
%
\begin{equation} \label{eq:pi_uc_system}
\dot{\vx} = \vf(t,\vx) + \vg(t,\vx) \varepsilon, \qquad \varepsilon \sim \mathcal{N}(\mathbf{0},\mathbf{\Sigma}), \quad \vx(t=s)=\vy
\end{equation}
%
Before we move on to the next section, we would like to give few insights into
the path integral formulation for optimal control. In this discussion we will
mainly use  equations~\eqref{eq:pi_optimal_controller} and
\eqref{eq:pi_uc_system}, however the same argument holds for the formulation in
equations~\eqref{eq:pi_original_optimal_controller} and \eqref{eq:uc_sde}.

According to equation~\eqref{eq:pi_optimal_controller1} in order to derive the
optimal control at time $s$ and state $\vy$, we should repeatedly forward
simulate the noise-driven system from that moment and point until the end of the
time horizon $t_f$. Then we should weight the first noise element of each sample
by $\alpha(\tau_{uc};s,\vy)$ which is defined as
%
\begin{equation}  \label{eq:pi_sample_weighting}
\alpha(\tau_{uc};s,\vy) = \sfrac{  \operatorname{e}^{-\frac{1}{\lambda}  \Big( \Phi(\vx(t_f))+ \int_{t_0}^{t_f} {q(t,\vx) \ dt} \Big) }  }    {\operatorname{E}_{\tau_{uc}} \left\{ \operatorname{e}^{-\frac{1}{\lambda}  \Big( \Phi(\vx(t_f))+ \int_{t_0}^{t_f} {q(t,\vx) \ dt} \Big) } \right\}} 
\end{equation}
%
Since in $\alpha(\tau_{uc};s,\vy)$ the accumulated cost is in the exponential,
this wighting will be almost zero for a costly trajectory and only a very small
portion of the samples with near optimal or optimal cost will have non-negligible
weights. However, the probability of generating optimal trajectories through the
noise-driven system (a.k.a. random walk) is very low. Therefore in order to be
able to estimate the optimal input, we need abundantly many samples. This issue
becomes even more severe in high dimensional problems, quickly to the point that
calculating the above exponential becomes intractable. In the next section, an
importance sampling scheme will be introduced which can boost the sampling
efficiency of the  Path Integral.
  
\vspace{8cm}
  
%
\section{Path Integral with Importance Sampling} \label{sec:PI_SI}
In order to make path integral sampling more efficient, we will use 
importance sampling. Before introducing the method, we will
briefly describe the idea behind importance sampling.

Assume the following expectation problem where $x$ is a random variable with
probability distribution $p(x)$ and $f(x)$ is an arbitrary deterministic
function.
%
\begin{equation*}
\operatorname{E}_{p}{[f(x)]} = \int_{-\infty}^{\infty}{f(x) \  p(x) dx}
\end{equation*}
%
We also assume that we have another random variable named $y$ with the
probability distribution $q(y)$. Lets assume that calculating the expectation of
an arbitrary function for this random variable is less costly than the previous
one. Is there a way to calculate $\operatorname{E}_{p}{[f(x)]}$, while we are only
sampling from $y$?

The answer is yes, as long as we can guarantee that $q(.)$ is non-zero everywhere
$p(.)$ is. In other words if the probability of extracting a particular value
of $x$ is non-zero, $y$ should also be able to have that value with some non-zero
probability. If this condition satisfies we can write
%
\begin{equation*}
\operatorname{E}_{p}{[f(x)]} = \operatorname{E}_{q}{[w(y) f(y)]}, \qquad w(y) = \frac{p(y)}{q(y)}
\end{equation*}
%
$w$ is called the importance sampling weighting. Proving this relation is
very simple, we just need to write the definition of the expectation. To do such,
we will start from the right hand side
%
\begin{align*}
\operatorname{E}_{q}{[w(y) f(y)]} &= \int_{-\infty}^{\infty}{w(y) f(y) q(y) \ dy}  \\
&= \int_{-\infty}^{\infty}{\frac{p(y)}{\cancel{q(y)}} f(y) \cancel{q(y)} \ dy} \\
&= \int_{-\infty}^{\infty}{p(y) f(y) \ dy} = \operatorname{E}_{p}{[f(x)]}
\end{align*}
%
Note that changing $y$ to $x$ is eligible since they are just dummy variables.

Now that we have introduced the idea of importance sampling, we will go back
to the path integral problem. First we will introduce importance sampling for
path integrals, then we will discuss how it can help to improve the sample
efficiency.

Lets assume that, for calculating the path integral expectations in
equation~\eqref{eq:pi_optimal_controller}, we use the following controlled system
dynamics instead of the uncontrolled dynamics (equation \ref{eq:pi_uc_system}).
%
\begin{equation} \label{eq:pi_c_system}
\dot{\vx} = \vf(t,\vx) + \vg(t,\vx) \left(u + \varepsilon\right), \qquad \varepsilon \sim \mathcal{N}(\mathbf{0},\mathbf{\Sigma}), \quad \vx(t=s)=\vy
\end{equation}
%
Now according to the importance sampling method, we need to incorporate the
importance sampling weighting into the expectation. This weighting should be 
defined as
%
\begin{equation*}
\frac{\mathbb{P}_{uc}(\tau \mid s, \vy)}{\mathbb{P}_{c}(\tau \mid s, \vy)} = 
\frac{\prod\limits_{i=0}^{N-1} {\mathcal{N} \Big(\vx(t_i) + \vf(t_i,\vx(t_i)) dt, \mathbf{\Xi}(t_i,\vx(t_i)) dt \Big)}}{\prod\limits_{i=0}^{N-1} {\mathcal{N} \Big(\vx(t_i) + \vf(t_i,\vx(t_i)) dt + \vg(t_i,\vx(t_i)) \vu(t_i) dt, \mathbf{\Xi}(t_i,\vx(t_i)) dt \Big)}}
\end{equation*}
%
where $\mathbb{P}_{c}$ is the probability distribution of the trajectory generated by the controlled system in equation~\eqref{eq:pi_c_system}. For the sake of simplicity, we will temporarily drop the time and state dependency of the functions. Therefore we will have
%
\begin{align*}
\frac{\mathbb{P}_{uc}(\tau \mid s, \vy)}{\mathbb{P}_{c}(\tau \mid s, \vy)} &= 
\prod\limits_{i=0}^{N-1} {\frac{ \mathcal{N} \Big(\vx_i + \vf_i dt, \mathbf{\Xi}_i dt \Big)}{\mathcal{N} \Big(\vx_i + \vf_i dt + \vg_i \vu_i dt, \mathbf{\Xi}_i dt \Big)}} \\
&= \prod\limits_{i=0}^{N-1} { \frac{ \exp\Big(-\frac{1}{2} \norm{\vx_{i+1}-\vx_i - \vf_i dt}^2_{\mathbf{\Xi}_i dt} \Big) }{ \exp\Big(-\frac{1}{2} \norm{\vx_{i+1} - \vx_i - \vf_i dt - \vg_i \vu_i dt}^2_{\mathbf{\Xi}_i dt} \Big) } }
\end{align*}
%
Since the trajectory is generated through the controlled dynamics, we know $d\vx_{i+1} = \vf_i dt + \vg_i \vu_i dt + \vg_i d\vw_i$. Hence we get
%
\begin{align*}
\frac{\mathbb{P}_{uc}(\tau \mid s, \vy)}{\mathbb{P}_{c}(\tau \mid s, \vy)} &= 
\prod\limits_{i=0}^{N-1} { \frac{ \exp\Big(-\frac{1}{2} \norm{\vg_i \vu_i dt + \vg_i d\vw_i}^2_{\mathbf{\Xi}_i dt} \Big) }{ \exp\Big(-\frac{1}{2} \norm{ \vg_i d\vw_i}^2_{\mathbf{\Xi}_i dt} \Big) } } \\
&= \prod\limits_{i=0}^{N-1} { \exp\Big( -\frac{1}{2} \norm{\vg_i \vu_i dt + \vg_i d\vw_i}^2_{\mathbf{\Xi}_i dt} + \frac{1}{2} \norm{ \vg_i d\vw_i}^2_{\mathbf{\Xi}_i dt}  \Big) } \\
&= \prod\limits_{i=0}^{N-1} { \exp\Big( -\frac{1}{2} \norm{\vg_i \vu_i dt}^2_{\mathbf{\Xi}_i dt}  -\cancel{\frac{1}{2} \norm{\vg_i d\vw_i}^2_{\mathbf{\Xi}_i dt}} - \vu_i^T \vg_i^T \mathbf{\Xi}_i^{-1} \vg_i d\vw_i + \cancel{\frac{1}{2} \norm{\vg_i d\vw_i}^2_{\mathbf{\Xi}_i dt}}  \Big) } \\
&= \prod\limits_{i=0}^{N-1} { \exp\Big( -\frac{1}{2} \vu_i^T \vg_i^T \mathbf{\Xi}_i^{-1} \vg_i \vu_i dt  - \vu_i^T \vg_i^T \mathbf{\Xi}_i^{-1} \vg_i d\vw_i \Big) } \\
&= \prod\limits_{i=0}^{N-1} { \exp\Big( -\frac{1}{2 \lambda} \vu_i^T \vR \vu_i dt  - \frac{1}{\lambda} \vu_i^T \vR d\vw_i \Big) } \\
&= \exp\Big( -\frac{1}{\lambda} \sum\limits_{i=0}^{N-1} { \frac{1}{2} \vu_i^T \vR \vu_i dt  + \vu_i^T \vR d\vw_i } \Big) \\
&=  \exp \Big( -\frac{1}{\lambda}  \displaystyle\int_{t_0}^{t_f} { \frac{1}{2} \vu^T \vR \vu dt + \vu^T \vR d\vw } \Big)
\end{align*}
%
Now if we multiply this importance sampling correction term to the expectations in equation~\eqref{eq:pi_optimal_controller}, we get
%
\begin{equation} 
\vu^*(s,\vy) = \frac{  \operatorname{E}_{\tau_{c}} \left\{ (\vu+\varepsilon) \  \operatorname{e}^{-\frac{1}{\lambda}  \Big( \Phi(\vx(t_f))+ \int_{t_0}^{t_f} {q(t,\vx) + \frac{1}{2} \vu^T \vR \vu \ dt + \vu^T \vR d\vw} \Big) } \right\} }    {\operatorname{E}_{\tau_{c}} \left\{ \operatorname{e}^{-\frac{1}{\lambda}  \Big( \Phi(\vx(t_f))+ \int_{t_0}^{t_f} {q(t,\vx) + \frac{1}{2} \vu^T \vR \vu \ dt + \vu^T \vR d\vw} \Big) } \right\}}
\end{equation} 
%
We have changed the $\tau_{uc}$ subscript to $\tau_c$ and substituted
$\varepsilon$ by $\vu + \varepsilon$. We can introduce the return of a trajectory
as
%
\begin{equation}
R(\tau;s,\vy) = \Phi(\vx(t_f))+ \int_{s}^{t_f} {\left(q(t,\vx) + \frac{1}{2} \vu^T \vR \vu\right) dt} + \int_{s}^{t_f} {\vu^T \vR d\vw} 
\end{equation}
%
Note that since the Brownian motion has a zero mean, the expectation of the
return (at initial time $t_0$ and initial state $\vx_0$) is equal to the cost
function of the policy $\vu$, i.e. $J = E{[R(\tau;t_0,\vx_0)]}$. Using the
return notation, the optimal control equation reduces to the following form
%
\begin{equation}  \label{eq:pi_is_optimal_controller}
\vu^*(s,\vy) = \vu(s,\vy) + \frac{  \operatorname{E}_{\tau_{c}} \left\{ \vvep(s) \  \operatorname{e}^{-\frac{1}{\lambda}  R(\tau;s,\vy) } \right\} }    {\operatorname{E}_{\tau_{c}} \left\{ \operatorname{e}^{-\frac{1}{\lambda}  R(\tau;s,\vy) } \right\}}
\end{equation} 


%
\section{Path Integral with Function Approximation} \label{sec:PI_FA}
The equation~\eqref{eq:pi_is_optimal_controller} indicates that in order to
calculate the optimal control at a specific time and state we must calculate
two expectations. In practice for a nonlinear system we estimate these
expectations through a Monte Carlo method. This means that we extract a
sufficiently big set of samples by forward simulating the controlled dynamics
from a given time and state. Then we estimate the expectations by a numerical
average over the samples. However in order to find the optimal policy, we need to
repeat this process for all the time steps in the period $[t_0,t_t]$ and at least
a subset of the state space. As you can imagine, this is typically quite a costly process.
On the other hand, we know that the final optimal control manifold is relatively
smooth (or at least we prefer to have a smooth approximation of it), which means
the estimated optimal control for a specific time and state could possibly be used
for its neighboring time steps and states. This idea can be included in the path
integral approach by using function approximation on the optimal control. Lets
assume that want to approximate the optimal control input through the
following linear model (linear w.r.t. the parameter vector)
%
\begin{equation}
u^*_i(s,\vy) = \vUpsilon_i^T(s,\vy) \vth_i^* + error
\end{equation}
%
where $u_i$ refers to the \textit{i}th control input. $\vUpsilon_i(s,\vy)$ is a
nonlinear basis function vector for the control input \textit{i} which can have
any arbitrary functionality of time and state. $\vth_i^*$ is the optimal
parameter vector. Calculating the optimal parameter vector for this linear model
introduces a linear regression problem. In order to solve the regression problem,
we must define an appropriate objective function. Here we will consider the
mean squared error criterion. The optimal parameter vector for each of the
$m$-control inputs can be calculated through the following optimization.
%
\begin{align}
\vth_i^* &= \argmax\limits_{\theta_i}{L(\vth_i)} \notag \\
&= \argmax\limits_{\vth_i}{ \int_{t_0}^{t_f}{{\int \frac{1}{2}\norm{u^*_i(s,\vy) - \vUpsilon_i^T(s,\vy) \vth_i}^2_2 \ p(s,\vy)d\vy} ds} }
\end{align}
%
where $p(s,\vy)$ is an arbitrary weighting function that has a unit integral
(therefore it can be considered as a probability distribution function). Since
the gradient of the optimal parameter vector should be zero, we can write
%
\begin{align}
 \frac{\partial L(\vth_i^*)}{\partial \vth_i} = \int_{t_0}^{t_f}{{\int \Big(u^*_i(s,\vy) - \vUpsilon_i^T(s,\vy) \vth_i^* \Big) \vUpsilon_i(s,\vy) \ p(s,\vy)d\vy} ds} = 0
\end{align}
%
Through multiplying and dividing the integrand by $\operatorname{E}_{\tau_{c}} \left\{ \operatorname{e}^{-\frac{1}{\lambda}  R(\tau;s,\vy) } \right\}$, we get
%
\begin{align}
 \int_{t_0}^{t_f}{{\int \frac{ \operatorname{E}_{\tau_{c}} \left\{ \operatorname{e}^{-\frac{1}{\lambda}  R(\tau;s,\vy) } \right\} }    {\operatorname{E}_{\tau_{c}} \left\{ \operatorname{e}^{-\frac{1}{\lambda}  R(\tau;s,\vy) } \right\}} \Big(u^*_i(s,\vy) - \vUpsilon_i^T(s,\vy) \vth_i^* \Big) \vUpsilon_i(s,\vy) \ p(s,\vy)d\vy} ds} = 0
\end{align}
%
We then push all of the terms inside of the nominator's
$\operatorname{E}_{\tau_{c}}\{.\}$. Notice that this operation is eligible
because the initial state $\vy$ is not a part of the expectation and is
assumed to be known.
%
\begin{equation}
 \int_{t_0}^{t_f}{{\int_{\Omega} \operatorname{E}_{\tau_{c}} \left\{\frac{  \operatorname{e}^{-\frac{1}{\lambda}  R(\tau;s,\vy) } }    {\operatorname{E}_{\tau_{c}} \left\{ \operatorname{e}^{-\frac{1}{\lambda}  R(\tau;s,\vy) } \right\}} \Big(u^*_i(s,\vy) - \vUpsilon_i^T(s,\vy) \vth_i^* \Big) \vUpsilon_i(s,\vy) \ p(s,\vy) \right\} d\vy} ds} = 0
\end{equation}
%
In order to shorten notation, we will show all of the expectations in integral
form and only use one integral sign, instead of three.
%
\begin{equation}
 \int {\frac{  \operatorname{e}^{-\frac{1}{\lambda}  R(\tau;s,\vy) } }    {\operatorname{E}_{\tau_{c}} \left\{ \operatorname{e}^{-\frac{1}{\lambda}  R(\tau;s,\vy) } \right\}} \Big(u^*_i(s,\vy) - \vUpsilon_i^T(s,\vy) \vth_i^* \Big) \vUpsilon_i(s,\vy) \ \mathbb{P}_{\tau_c}(\tau\mid s, \vy) p(s,\vy) \  d\tau d\vy ds} = 0
\end{equation}
%
In the next step, we will add and subtract the terms $u_i(s,\vy) + \varepsilon(s)$.
%
\begin{align}
 \int \frac{  \operatorname{e}^{-\frac{1}{\lambda}  R(\tau;s,\vy) } }    {\operatorname{E}_{\tau_{c}} \left\{ \operatorname{e}^{-\frac{1}{\lambda}  R(\tau;s,\vy) } \right\}} \Big(u^*_i - u_i - \varepsilon + u_i + \varepsilon - \vUpsilon_i^T \vth_i^* \Big) \vUpsilon_i(s,\vy) \ \mathbb{P}_{\tau_c}(\tau\mid s, \vy) p(s,\vy) d\tau d\vy ds = 0
\end{align}
%
We break this integral into two integrals as follows
%
\begin{align}
 \int &{\frac{  \operatorname{e}^{-\frac{1}{\lambda}  R(\tau;s,\vy) } }    {\operatorname{E}_{\tau_{c}} \left\{ \operatorname{e}^{-\frac{1}{\lambda}  R(\tau;s,\vy) } \right\}} \Big(u^*_i(s,\vy) -u_i(s,\vy) - \varepsilon \Big) \vUpsilon_i(s,\vy) \ \mathbb{P}_{\tau_c}(\tau\mid s, \vy) p(s,\vy) d\tau d\vy ds} + \notag\\
 &\int {\frac{  \operatorname{e}^{-\frac{1}{\lambda}  R(\tau;s,\vy) } }    {\operatorname{E}_{\tau_{c}} \left\{ \operatorname{e}^{-\frac{1}{\lambda}  R(\tau;s,\vy) } \right\}} \Big(u_i(s,\vy) + \varepsilon - \vUpsilon_i^T(s,\vy) \vth_i^* \Big) \vUpsilon_i(s,\vy) \ \mathbb{P}_{\tau_c}(\tau\mid s, \vy) p(s,\vy) d\tau d\vy ds} = 0
\end{align}
%
For the first integral, we will first integrate it with respect to trajectory
$\tau$ and then use equation~\eqref{eq:pi_is_optimal_controller}.
%
\begin{align*}
 & \int {\frac{  \operatorname{e}^{-\frac{1}{\lambda}  R(\tau;s,\vy) } }    {\operatorname{E}_{\tau_{c}} \left\{ \operatorname{e}^{-\frac{1}{\lambda}  R(\tau;s,\vy) } \right\}} \Big(u^*_i(s,\vy) -u_i(s,\vy) - \varepsilon \Big) \vUpsilon_i(s,\vy) \ \mathbb{P}_{\tau_c}(\tau\mid s, \vy) p(s,\vy) d\tau d\vy ds} = \notag\\
 & \int { \left(u^*_i(s,\vy) - u_i(s,\vy) - \frac{  \operatorname{E}_{\tau_{c}} \left\{\varepsilon \operatorname{e}^{-\frac{1}{\lambda}  R(\tau;s,\vy) } \right\} }    {\operatorname{E}_{\tau_{c}} \left\{ \operatorname{e}^{-\frac{1}{\lambda}  R(\tau;s,\vy) } \right\}} \right)  \vUpsilon_i(s,\vy) \ (\tau\mid s, \vy) p(s,\vy) d\vy ds} = 0
\end{align*}
%
By substituting this result back into the previous equation we get
%
\begin{equation}
 \int {\frac{  \operatorname{e}^{-\frac{1}{\lambda}  R(\tau;s,\vy) } }    {\operatorname{E}_{\tau_{c}} \left\{ \operatorname{e}^{-\frac{1}{\lambda}  R(\tau;s,\vy) } \right\}} \Big(u_i(s,\vy) + \varepsilon - \vUpsilon_i^T(s,\vy) \vth_i^* \Big) \vUpsilon_i(s,\vy) \ \mathbb{P}_{\tau_c}(\tau\mid s, \vy) p(s,\vy) d\tau d\vy ds} = 0
\end{equation}
%
which is equivalent to the following optimization problem
%
\begin{equation} \label{eq:pi_is_fa_optimal_controller_original}
 \vth_i^* = \argmin_{\vth_i}{\int {\frac{  \operatorname{e}^{-\frac{1}{\lambda}  R(\tau;s,\vy) } }    {\operatorname{E}_{\tau_{c}} \left\{ \operatorname{e}^{-\frac{1}{\lambda}  R(\tau;s,\vy) } \right\}} \norm{\vUpsilon_i^T(s,\vy) \vth_i - u_i(s,\vy) - \varepsilon}^2_2 \ \mathbb{P}_{\tau_c}(\tau\mid s, \vy) p(s,\vy) d\tau d\vy ds}}
\end{equation}
%
If we use the same function approximation model for $u_i(s,\vy)$ and $u_i(s,\vy) \approx \vUpsilon_i^T(s,\vy) \vth_{i,c}$, we get
%
\begin{equation} \label{eq:pi_is_fa_optimal_controller}
 \vth_i^* = \vth_{i,c} + \argmin_{\Delta \vth_i}{\int {\frac{  \operatorname{e}^{-\frac{1}{\lambda}  R(\tau;s,\vy) } }    {\operatorname{E}_{\tau_{c}} \left\{ \operatorname{e}^{-\frac{1}{\lambda}  R(\tau;s,\vy) } \right\}} \norm{\vUpsilon_i^T(s,\vy) \Delta \vth_i - \varepsilon}^2_2 \ \mathbb{P}_{\tau_c}(\tau\mid s, \vy) p(s,\vy) d\tau d\vy ds}}
\end{equation}
%
Equation~\eqref{eq:pi_is_fa_optimal_controller_original} or
\eqref{eq:pi_is_fa_optimal_controller} introduce a method to blend the function
approximation and optimal control problems into a single optimization problem.
In the next section, we will introduce the general path integral  algorithm which
uses importance sampling and function approximation.


%
\section{General Path Integral Algorithm}
In this section, we will present the path integral general algorithm. In this
algorithm we will use all the components that we already have introduced in the
previous sections. Before putting things all to gather, we will describe the
reason behind each of the component separately.

\paragraph{Importance Sampling} As discussed previously, the original path
integral algorithm requires that the samples are extracted from the uncontrolled
system. Therefore, estimating the optimal control through a Monte Carlo method
will be extremely inefficient. However by using the Importance Sampling scheme
introduced in \sref{sec:PI_SI}, we can implement an incremental method to
estimate the optimal control which is more sample efficient. 

In this approach, we can start the sampling with a sophisticated guess
of the optimal control. Note that this is optional,though, and we could also start from the
uncontrolled system.In each iteration of the algorithm, we use our
latest guess of the optimal control to extract a batch of samples. Using this
batch of samples, we can improve our estimation of the optimal control. Our sampling efficiently inherently improves at the same time, since, as
our estimation improves, we sample an the area with lower accumulated cost and
therefore the sample weighings, $\alpha(\tau;s,\vy)$ (equation
\ref{eq:pi_sample_weighting}), will have more significant values. It can be shown
that if we are in the $\epsilon$-vicinity of the optimal solution the sample
efficiency will improve linearly with $\epsilon$.


\paragraph{Function Approximation} The original path integral theorem introduces
a sampling method for estimating the optimal control at a specific time and
state. Therefore for estimating the optimal control in a given time period and some subspace of the state space, we should repeat the estimation individually
for every point. In \sref{sec:PI_FA}, we introduced a function
approximation scheme in which the estimated optimal control for a single point
generalizes to its neighboring area. Another advantage of function approximation
is the introduction of $p(s,\vy)$ (the weighting function of MSE). For example,
assume we have chosen $p(s,\vy)$ as the probability distribution of the state under
the latest estimation of the optimal control. In this case, the function
approximation will be more precise in the area more likely to be visited
using the optimal policy.

Algorithm~\ref{alg:gpi} shows the General Path Integral Algorithm which uses
importance sampling and function approximation. 

\begin{algorithm}[tpb] \caption{General Path Integral Algorithm} \label{alg:gpi}
\begin{algorithmic} 
\State \textbf{given}
\State \hspace{4mm} The cost function: 
\State \hspace{8mm} $J = \Phi(\vx(t_f))+ \int_{s}^{t_f} {\left(q(t,\vx) + \frac{1}{2} \vu^T \vR \vu\right) dt}$
\State \hspace{4mm} A PDF defining the quality of approximation of optimal control at each time-state pair: $p(t,\vx)$
\State \hspace{4mm} An initial policy and a Linear Model: $\vu(t,\vx) = [u_i(t,\vx)] = [\vUpsilon^T_i(t,\vx) \vth_i]$
\Repeat{}
\State (a) Randomly choose a time-state pair from $p(t,\vx)$: $(s,\vy)$
\State (b) Forward simulate the controlled system for $K$ different rollouts: $\{ \tau^k \}_{k=1}^K$ 
\State \hspace{8mm} $\dot{\vx} = \vf(t,\vx) + \vg(t,\vx) \left(\vu + \vvep \right) $ 
\State \hspace{8mm} $ \vu(t,\vx) = [\vUpsilon^T_i(t,\vx) \vth_i], \ \vvep \sim \mathcal{N}(\mathbf{0},\mathbf{\Sigma}),\ \vx(t=s)=\vy$ 
\State (c) Calculate the return for each rollout: $\{ R^k \}_{k=1}^K$
\State \hspace{8mm} $R(\tau;s,\vy) = \Phi(\vx(t_f))+ \int_{s}^{t_f} {\left(q(t,\vx) + \frac{1}{2} \vu^T \vR \vu\right) dt} + \int_{s}^{t_f} {\vu^T \vR d\vw}$
\State (d) Calculate $\{\alpha^k\}_{k=1}^K$ 
\State \hspace{8mm} $\alpha^k(s,\vy) = \sfrac{ \exp (-\frac{1}{\lambda} R^k) }    {\frac{1}{K} \sum\limits_{j=1}^{K} \exp
(-\frac{1}{\lambda}  R^j) }$
\State (e) Solve the following linear regression problem for each control input $i$:
\State \hspace{8mm} $\Delta \vth_i = \argmin{\sum\limits_{k=1}^{K} {\alpha^k \norm{\vUpsilon_i^T(s,\vy) \Delta \vth_i - \varepsilon^k_i(s)}^2_2 }}$
\State (f) Update the parameter vector for each control input $i$:
\State \hspace{8mm} $\vth_i \leftarrow \vth_i + \omega \Delta \vth_i$
\Until{convergence}
\end{algorithmic} 
\end{algorithm}

 
%
\section{PI2 Algorithm: Time-dependent Policy}
The Policy Improvement Path Integral algorithm (PI2) is a variant of General Path
Integral algorithm. PI2 is an instance of a sample-based reinforcement learning
algorithm that can retrieve trajectory samples directly from the real
environment i.e. the real system. In this section, we will derive the PI2
algorithm from the General Path Integral algorithm.

Originally the PI2 algorithm was developed for optimizing parameterized,
time-dependent policies. The time-dependent policy can be either a parameterized
dynamical system like Dynamic Movement Primitives (DMPs) or simply a function
approximation of the control input like the one in
equation~\eqref{eq:pi2_t_policy}. The essential requirements for the algorithm are linearity w.r.t
the parameter vector, and the usage of time-dependent basis functions. In this section,
we will use function-approximation policies since it will later give us the
opportunity to extend the PI2 algorithm to more general polices that are
functions of time and state.
%
\begin{align} \label{eq:pi2_t_policy}
u_i(t) &= \vUpsilon^T(t) \vth_i \notag \\
\vUpsilon(t) &= \big[ \Upsilon_n(t) \big]_{N \times 1} =
\left[ e^{-\frac{1}{2}\frac{(t-\mu_n)^2}{\sigma_{n}^{2}}} \right]_{N \times 1}
\end{align}
%
In this equation, $u_i$ refers to the $i$th control input and $\vUpsilon$ is
a time-dependent basis function. Each element of $\Upsilon$ (denoted by
$\Upsilon_n$) is a bell-shape function with a mean and variance, $\mu_n$ and
$\sigma^2_n$ respectively. The dimension of the parameter vector as well as the
basis function vector is $N$.

In order to derive PI2 from the General Path Integral algorithm, we should make
the following assumptions:
%
\begin{enumerate}
\item The weighting function of MSE, $p(t,\vx)$, is assumed to be the probability
distribution of the state under the latest estimation of the optimal control.
Therefore the rollout trajectory's states are considered to be extracted from
$p(t,\vx)$.
%
\item The return function, $R(\tau;s,\vy)$, won't be a function of state if the
system has been initialized from a similar initial condition. An immediate result
of this assumption is that $\alpha^k(s,\vy)$ is only a function of time i.e.
$\alpha^k(s)$. Therefore for a batch of trajectories extracted from a similar
initial condition, $\alpha^k(s)$ can be estimated for each time step by the
following.
%
\begin{equation}
\alpha^k(s) = \frac{ \exp (-\frac{1}{\lambda} R^k(s)) }    {\frac{1}{K} \sum\limits_{j=1}^{K} \exp
(-\frac{1}{\lambda}  R^j(s) ) }
\end{equation}
%
Notice that in contrast to the general path integral algorithm, where we are
required to estimate $\alpha^k(s,\vy)$ by extracting trajectories starting from
$(s,\vy)$, we can use trajectories with different state values but
the same time indexes to estimate $\alpha$. Therefore, if we have a batch of
trajectories that are generated from similar initial conditions, we can estimate
$\alpha$ for all of the states and over the given time horizon, $[t_0,t_f]$.
%
\item The basis function vector for all of the control inputs is the same. Hence we
will drop the $i$ subscript of the basis function as $[u_i(t)]=[\vUpsilon^T(t)
\vth_i]$.
%
\item Instead of adding noise to the control input, the noise is added
directly to the parameter vector. Therefore, the input noise can be expressed as
$\vvep_i = \vUpsilon(t) \vep_i$, where $\vep_i$ is the noise that is added to the
parameter vector of the $i$th control input.
%
\item The PI2 regression problem should be modified as follows
%
\begin{equation}
\Delta \vth_i = \argmin{\sum\limits_{s=t_0}^{t_f}{\sum\limits_{k=1}^{K} {\alpha^k(s) \norm{\vUpsilon_i^T(s) \Delta \vth_i - \varepsilon^k_i(s)}^2_2 }}}
\end{equation}
%
In contrast to the General Path Integral Algorithm, PI2 assumes that samples
are extracted over the entire time horizon, not only for a single time step.
Therefore, the regression problem should be over all of the sampled trajectories as well as all of the sub-trajectories of each individual trajectory, where a sub-trajectory is a portion of a trajectory starting from some time $s$ until the end of the time horizon (as was illustrated in \sref{sec:mc_exploring_starts}).

In order to solve this regression problem, PI2 breaks it into two separate
optimizations. In doing so, it is assumed that the 
the regression error is zero mean over the samples. In this method, the
optimization is first solved for each time step separately. Therefore the first
optimization will find a time-dependent parameter vector increment that has the
minimum error over the rollouts at each time step. In the second optimization, we find a parameter vector increment that approximates the time-dependent one.

The first optimization is defined as follows for each time step $s$
%
\begin{equation} \label{eq:pi2_regression_inner}
\Delta \vth_i^*(s) = \argmin{\sum\limits_{k=1}^{K} {\alpha^k(s) \norm{\vUpsilon_i^T(s) \Delta \vth_i - \varepsilon^k_i(s)}^2_2 }}
\end{equation}
%
In this optimization, all of the regressors are the same. Therefore in order to find
the solution to this problem, we should use the right inverse which will give a
solution with the minimum-norm $\Delta \vth_i^*(s)$
%
\begin{equation} \label{eq:pi2_regression_inner_sol1}
\Delta \vth_i^*(s) = \sum\limits_{k=1}^{K} { \alpha^k(s) \frac{\vUpsilon_i(s)}{\vUpsilon_i^T(s) \vUpsilon_i(s)} \varepsilon^k_i(s) }
\end{equation}
%
If we use the fourth assumption that the noise is directly added to the parameter
vector, we get
\begin{equation} \label{eq:pi2_regression_inner_sol2}
\Delta \vth_i^*(s) = \sum\limits_{k=1}^{K} { \alpha^k(s) \frac{\vUpsilon_i(s) \vUpsilon_i^T(s)}{\vUpsilon_i^T(s) \vUpsilon_i(s)} \vep^k_i(s) }
\end{equation}
%
The second optimization for finding the optimal $\Delta\vth_{i}^*$ is defined in
equation~\eqref{eq:pi2_regression_outer}. The index $n$ refers to the $n$th
element of the vector $\Delta\vth_{i}^*=[\Delta\theta_{i,n}^*]$
%
\begin{equation} \label{eq:pi2_regression_outer}
\Delta \theta_{i,n}^* = \argmin\limits_{\Delta \theta_{i,n}}{\sum\limits_{s=t_0}^{t_f}{  ( \Delta \theta_{i,n} - \Delta \theta_{i,n}^*(s) )^2 \Upsilon_n(s) }}
\end{equation}
%
$\Upsilon_n(t)$ is the $n$th element of the basis function vector $\vUpsilon(t)$. 
The solution to this optimization can be easily calculated as
%
\begin{equation}
\Delta \theta_{in}^* = \frac{ \sum\limits_{t=t_0}^{t_f}{\Delta \theta_{in}^*(s) \Upsilon_n(s)} }{ \sum\limits_{t=t_0}^{t_f}{\Upsilon_n(s)} }
\end{equation}
%
By using element-wise multiplication and division and replacing the summation
with an integral, we can also write
%
\begin{equation} \label{eq:pi2_regression_outer_sol}
\Delta \vth_{i}^* = \left({ \int\limits_{t_0}^{t_f}{\Delta \vth_{i}^*(s) \circ \vUpsilon(s) ds} }\right)  \cdot\bigg/ { \int\limits_{t_0}^{t_f} {\vUpsilon(s) ds} }
\end{equation}
%
where $\circ$ and $\cdot/$ are element-wise multiplication and division.
%
\end{enumerate}
%
Using these assumptions, we can derive PI2 from the General Path Integral
algorithm. The complete algorithm is given as
Algorithm~\ref{alg:pi2_time_policy}. Notice that in PI2, we do not need
to artificially initialize the system at random points $(s,\vy)$ according to
$p(s,\vy)$. Therefore this algorithm is a sample-based
reinforcement learning algorithm and can be used to learn the optimal policy through
samples that are generated directly from the real physical system.

\newpage

\begin{algorithm}[H] \caption{PI2 Algorithm for time-dependent policy} \label{alg:pi2_time_policy}
\begin{algorithmic}
\State \textbf{given}
\State \hspace{4mm} The cost function: 
\State \hspace{8mm} $J = \Phi(\vx(t_f))+ \int_{t_0}^{t_f} {\left(q(t,\vx) + \frac{1}{2} \vu^T \vR \vu\right) dt}$
\State \hspace{4mm} A linear model for function approximation: $\vu(t) = [u_i(t)] = [\vUpsilon^T(t) \vth_i]$
\State \hspace{4mm} Initialize $[\vth_i]$ with a sophisticated guess 
\State \hspace{4mm} Initialize exploration noise standard deviation: $c$

\Repeat
\State Create $K$ rollouts of the system with the perturbed parameter $[\vth_i] +
[\vep_i], \quad \vep_i \sim \mathcal{N} (\mathbf{0},c^2\vI)$
\For{the $i$th control input}
\For{each time, s}
\State Calculate the Return from starting time $s$ for the $k$th rollout:
\State \hspace{4mm} $R(\tau^k(s)) = \Phi(\vx(t_f)) + \int_{s}^{t_f} {\left(q(t,\vx) + \frac{1}{2} \vu^T \vR \vu\right) dt}$
\State Calculate $\alpha$ from starting time $s$ for the $k$th rollout:
\State \hspace{4mm} $\alpha^k(s) = \sfrac{ \exp ( -\frac{1}{\lambda}R(\tau^k(s)) ) }{
\sum_{k=1}^{K}{ \exp( -\frac{1}{\lambda}R(\tau^k(s)) ) } }$
\State Calculate the time varying parameter increment $\Delta \vth_{i}(s)$:
\State \hspace{4mm} $\Delta \vth_{i}(s) = \sum_{k=1}^{K}{\alpha^k(s) \frac{\vUpsilon(s) \vUpsilon^T(s)}{ \vUpsilon^T(s) \vUpsilon(s)} \vep^k_i(s)}$
\EndFor
\State Time-averaging the parameter vector
\State \hspace{4mm} $\Delta \vth_{i} = \left({ \int\limits_{t_0}^{t_f}{\Delta \vth_{i}(s) \circ \vUpsilon(s) ds} }\right) \cdot\bigg/ { \int\limits_{t_0}^{t_f} {\vUpsilon(s) ds} }$
\State Update parameter vector for control input $i$, $\vth_i$:
\State \hspace{4mm} $\vth_i \leftarrow \vth_i + \Delta \vth_i$
\EndFor
\State Decrease c for noise annealing
\Until{maximum number of iterations}
\end{algorithmic}
\end{algorithm}

%
\section{PI2 Algorithm: Feedback Gain Learning}
In a first attempt to tailor the PI2 algorithm to more general policies, we will introduce a method to
learn a linear time-varying feedback gain. Consider the following tracking problem
%
\begin{equation}
\begin{cases}
\dot{\vx} = \vf(t,\vx) + \vg(t,\vx)\vu \\
\vu = \vK^T(t)(\vx-\vx_{ref})
\end{cases}
\end{equation}
%
For now, we will assume that the control input dimension is one. If we substitute
the linear feedback controller back into the system dynamics, we will get
%
\begin{equation}
\dot{\vx} = \vf(t,\vx) + \vg(t,\vx)  (\vx-\vx_{ref})^T \vK(t) \\
\end{equation}
%
According to this equation, we can assume a new system with $\vK(t)$ as its
control input. Considering this new system, we can use
Algorithm~\ref{alg:pi2_time_policy} to learn the time varying feedback gains.
This method can be easily extended to a system with multiple control inputs. The
learning algorithm in this case will assume a system that has as many inputs as
the total number of gains. In other words if the dimensions of the state and control
input vectors are $\dim[\vx]$ and $\dim[\vu]$ respectively, the dimension of
control input from the perspective of PI2 will be $\dim[\vx] \times \dim[\vu]$.

In the next section, we will introduce a more general algorithm which will
learn both time-dependent policies and the feedback gains simultaneously.

%
\section{PI2 Algorithm: General Algorithm}
In this section, the General PI2 algorithm will be modified to allow
policies with linear state dependency and a nonlinear time dependency to be learned. An
instance of such a policy is as follows
%
\begin{align} \label{eq:pi2_t_x_policy}
u_i(t,\vx) &= \operatorname{grand\,sum}{\left[\bar{\vUpsilon}(t,\vx) \circ \vth_i\right]}  \notag\\
\bar{\vUpsilon}(t,\vx) &= \vUpsilon(t) \begin{bmatrix} 1 & \vx^T \end{bmatrix} =
\left[ e^{-\frac{1}{2}\frac{(t-\mu_n)^2}{\sigma_{n}^{2}}} \begin{bmatrix} 1 & \vx^T \end{bmatrix}
\right]_{N \times (1+\dim{[\vx]})}
\end{align}
%
The $\operatorname{grand\,sum}$ operator calculates the sum of all the elements
in a matrix and $\circ$ is the element-wise multiplication.  $\vth_i$ is a $N
\times (1+\dim{[\vx]})$ parameter matrix for $i$th control input approximation.
$\bar{\vUpsilon}(t,\vx)$ is the basis function matrix of the same size as
$\vth_i$. Finally $\vUpsilon(t)$ is defined as in equation~\eqref{eq:pi2_t_policy}.

By setting the parameters which are multiplied by the states to zero, this policy
reduces to the time varying policy primarily introduced in the
equation~\eqref{eq:pi2_t_policy}. Using the same argument from the previous
section we can assume that the state dependent segment of the policy is part of
the system dynamics and PI2 will be used to learn the time-varying gains. Based
on the policy in equation~\eqref{eq:pi2_t_x_policy}, we can assume that these
gains are sufficiently approximated by the using time-dependent basis function, $\vUpsilon(t)$.
The compete algorithm is given in Algorithm~\ref{alg:general_pi2}.


\begin{algorithm}[tpb] \caption{General PI2 Algorithm} \label{alg:general_pi2}
\begin{algorithmic}
\State \textbf{given}
\State \hspace{4mm} The cost function: 
\State \hspace{8mm} $J = \Phi(\vx(t_f))+ \int_{t_0}^{t_f} {\left(q(t,\vx) + \frac{1}{2} \vu^T \vR \vu\right) dt}$
\State \hspace{4mm} A linear model for function approximation: $\vu(t,\vx) = [u_i(t,\vx)] = \left[\operatorname{grand\,sum}{[\bar{\vUpsilon}(t,\vx) \circ \vth_i]} \right]$
\State \hspace{4mm} Initialize $\{\vth_i\}$ with a sophisticated guess 
\State \hspace{4mm} Initialize exploration noise standard deviation: $c$

\Repeat
\State Create $K$ rollouts of the system with the perturbed parameter $ \{\vth_i\} +
\{\vep_i\}, \  \{\vep_{i,j}\} \sim \mathcal{N} (\mathbf{0},c^2\vI)$
\For{the $i$th control input}
\For{each time, s}
\State Calculate the Return from starting time $s$ for the $k$th rollout:
\State \hspace{4mm} $R(\tau^k(s)) = \Phi(\vx(t_f)) + \int_{s}^{t_f} {\left(q(t,\vx) + \frac{1}{2} \vu^T \vR \vu\right) dt}$
\State Calculate $\alpha$ from starting time $s$ for the $k$th rollout:
\State \hspace{4mm} $\alpha^k(s) = \sfrac{ \exp ( -\frac{1}{\lambda}R(\tau^k(s)) ) }{
\sum_{k=1}^{K}{ \exp( -\frac{1}{\lambda}R(\tau^k(s)) ) } }$
\State Calculate the time varying parameter increment $\Delta \vth_{i}(s)$:
\State \hspace{4mm} $\Delta \vth_{i}(s) = \sum_{k=1}^{K}{\alpha^k(s) \frac{\vUpsilon(s) \vUpsilon^T(s)}{ \vUpsilon^T(s) \vUpsilon(s)} \vep^k_i(s)}$
\EndFor
\For{the $j$th column of $\Delta \vth_{i}$ matrix, $\Delta \vth_{i,j}$}
\State Time-averaging the parameter vector
\State \hspace{4mm} $\Delta \vth_{i,j} = \left({ \int\limits_{t_0}^{t_f}{\Delta \vth_{i,j}(s) \circ \vUpsilon(s) ds} }\right) \cdot\bigg/ { \int\limits_{t_0}^{t_f} {\vUpsilon(s) ds} }$
\EndFor
\State Update parameter vector for control input $i$, $\vth_i$:
\State \hspace{4mm} $\vth_i \leftarrow \vth_i + \Delta \vth_i$
\EndFor
\State - Decrease c for noise annealing
\Until{maximum number of iterations}
\end{algorithmic}
\end{algorithm}


==> misc/abstract.tex <==
\thispagestyle{empty}
\chapter*{Abstract}

This is my abstract.

==> misc/acknowledgements.tex <==
\thispagestyle{empty}
\chapter*{Acknowledgement}

Thank you.
